Exploiting Pilot Mixtures in Coded Random Access

The construction of preamble sequences for channel estimation by superposition of orthogonal pilots can improve performance of massive grant-free uplink from machine-type devices. In this letter, a technique is proposed to obtain full benefit from these "pilot mixtures" in presence of a base station with a massive number of antennas. The proposed technique consists of combining pilot mixtures with an intra-slot successive interference cancellation (SIC) algorithm, referred to as inner SIC, to increase the number of decoded messages per slot. In framed systems, the synergic effect of inner SIC and of an outer SIC algorithm across slots, typical of coded random access protocols, allows achieving a very high reliability with a low number of packet replicas per active user.

==> Figures/table_VarM.tex <==
\begin{table}[t]
    \centering
    \caption{Optimum asymptotic thresholds constrained to $\Lambda'(1) = 3.0$ versus the number of antennas $M$. Optimum distribution $\Lambda(x) = x^3$ in all cases, $N_\mathrm{P} = 64$, $t = 10$, $N_\mathrm{D} = 256$.}
    %Asymptotic thresholds analysis varying the number of antennas $M$. The analysis is conducted adopting $\Lambda^{\prime}(1) = 3.0$, the corresponding optimal distribution $\Lambda(x) = x^3$, $N_\mathrm{P} = 64$, $t = 10$, $N_\mathrm{D} = 256$.}
    \label{tab:VarM}
    \small
    \begin{tabular}{ccc}
        \toprule
        \rowcolor[gray]{.95}
        $M$ & $G^*$ & $G^* / M$\\
        \midrule
        %$1$   & $0.0159$ & $0.0159$ \\
        %\rowcolor[gray]{.95}
        %$2$   & $0.0159$ & $0.0079$ \\
        %$4$   & $0.0258$ & $0.0065$ \\
        %\rowcolor[gray]{.95}
        $8$   & $0.1356$ & $0.0169$ \\
        $16$  & $0.4409$ & $0.0276$ \\
        %\rowcolor[gray]{.95}
        $32$  & $1.0562$ & $0.0330$ \\
        $64$  & $2.0778$ & $0.0325$ \\
        %\rowcolor[gray]{.95}
        $128$ & $3.8167$ & $0.0298$ \\
        $256$ & $6.9909$ & $0.0273$ \\
        \bottomrule
    \end{tabular}
\end{table}
